UP-dROM : Uncertainty-Aware and Parametrised dynamic Reduced-Order Model, application to unsteady flows

Reduced order models (ROMs) play a critical role in fluid mechanics by providing low-cost predictions, making them an attractive tool for engineering applications. However, for ROMs to be widely applicable, they must not only generalise well across different regimes, but also provide a measure of confidence in their predictions. While recent data-driven approaches have begun to address nonlinear reduction techniques to improve predictions in transient environments, challenges remain in terms of robustness and parametrisation. In this work, we present a nonlinear reduction strategy specifically designed for transient flows that incorporates parametrisation and uncertainty quantification. Our reduction strategy features a variational auto-encoder (VAE) that uses variational inference for confidence measurement. We use a latent space transformer that incorporates recent advances in attention mechanisms to predict dynamical systems. Attention's versatility in learning sequences and capturing their dependence on external parameters enhances generalisation across a wide range of dynamics. Prediction, coupled with confidence, enables more informed decision making and addresses the need for more robust models. In addition, this confidence is used to cost-effectively sample the parameter space, improving model performance a priori across the entire parameter space without requiring evaluation data for the entire domain.

==> biblio.tex <==

@article{MENIER2023115985,
title = {CD-ROM: Complemented Deep - Reduced order model},
journal = {Computer Methods in Applied Mechanics and Engineering},
volume = {410},
pages = {115985},
year = {2023},
issn = {0045-7825},
doi = {https://doi.org/10.1016/j.cma.2023.115985},
url = {https://www.sciencedirect.com/science/article/pii/S0045782523001081},
author = {Emmanuel Menier and Michele Alessandro Bucci and Mouadh Yagoubi and Lionel Mathelin and Marc Schoenauer},
keywords = {Reduced order models, Deep learning, Neural ODE, Computational fluid dynamics},
abstract = {Model order reduction through the POD-Galerkin method can lead to dramatic gains in terms of computational efficiency in solving physical problems. However, the applicability of the method to non linear high-dimensional dynamical systems such as the Navier–Stokes equations has been shown to be limited, producing inaccurate and sometimes unstable models. This paper proposes a deep learning based closure modeling approach for classical POD-Galerkin reduced order models (ROM). The proposed approach is theoretically grounded, using neural networks to approximate well studied operators. In contrast with most previous works, the present CD-ROM approach is based on an interpretable continuous memory formulation, derived from simple hypotheses on the behavior of partially observed dynamical systems. The final corrected models can hence be simulated using most classical time stepping schemes. The capabilities of the CD-ROM approach are demonstrated on two classical examples from Computational Fluid Dynamics, as well as a parametric case, the Kuramoto–Sivashinsky equation.}
}

@article{DMD,
author = {Schmid, Peter and Sesterhenn, Jörn},
year = {2008},
month = {11},
pages = {},
title = {Dynamic Mode Decomposition of numerical and experimental data},
volume = {656},
journal = {Journal of Fluid Mechanics},
doi = {10.1017/S0022112010001217}
}

@article{DMDLimits,
author = {Wu, Ziyou and Brunton, Steven and Revzen, Shai},
year = {2021},
month = {12},
pages = {},
title = {Challenges in dynamic mode decomposition},
volume = {18},
journal = {Journal of The Royal Society Interface},
doi = {10.1098/rsif.2021.0686}
}

@article{doi:10.1137/21M1401243,
author = {Brunton, Steven L. and Budi\v{s}i\'{c}, Marko and Kaiser, Eurika and Kutz, J. Nathan},
title = {Modern Koopman Theory for Dynamical Systems},
journal = {SIAM Review},
volume = {64},
number = {2},
pages = {229-340},
year = {2022},
doi = {10.1137/21M1401243},

URL = { 
    
        https://doi.org/10.1137/21M1401243
},
eprint = { 
    
        https://doi.org/10.1137/21M1401243
}
,
    abstract = { The field of dynamical systems is being transformed by the mathematical tools and algorithms emerging from modern computing and data science. First-principles derivations and asymptotic reductions are giving way to data-driven approaches that formulate models in operator-theoretic or probabilistic frameworks. Koopman spectral theory has emerged as a dominant perspective over the past decade, in which nonlinear dynamics are represented in terms of an infinite-dimensional linear operator acting on the space of all possible measurement functions of the system. This linear representation of nonlinear dynamics has tremendous potential to enable the prediction, estimation, and control of nonlinear systems with standard textbook methods developed for linear systems. However, obtaining finite-dimensional coordinate systems and embeddings in which the dynamics appear approximately linear remains a central open challenge. The success of Koopman analysis is due primarily to three key factors: (1) there exists rigorous theory connecting it to classical geometric approaches for dynamical systems; (2) the approach is formulated in terms of measurements, making it ideal for leveraging big data and machine learning techniques; and (3) simple, yet powerful numerical algorithms, such as the dynamic mode decomposition (DMD), have been developed and extended to reduce Koopman theory to practice in real-world applications. In this review, we provide an overview of modern Koopman operator theory, describing recent theoretical and algorithmic developments and highlighting these methods with a diverse range of applications. We also discuss key advances and challenges in the rapidly growing field of machine learning that are likely to drive future developments and significantly transform the theoretical landscape of dynamical systems. }
}

@article{Gupta2023MoriZwanzigLS,
  title={Mori-Zwanzig latent space Koopman closure for nonlinear autoencoder},
  author={Priyam Gupta and Peter J. Schmid and Denis Sipp and Taraneh Sayadi and Georgios Rigas},
  journal={ArXiv},
  year={2023},
  volume={abs/2310.10745},
  url={https://api.semanticscholar.org/CorpusID:264172182}
}

@article {ILED,
	title = {Interpretable Learning of Effective Dynamics for multiscale systems},
	year = {Submitted},
	url = {https://arxiv.org/abs/2309.05812},
	author = {Menier, Emmanuel and Kaltenbach, Sebastian and Yagoubi, Mouadh and Schoenauer, Marc and Koumoutsakos, Petros}
}

@article{SLT,
author = {Shokar, Ira and Kerswell, Rich and Haynes, Peter},
year = {2024},
month = {06},
pages = {},
title = {Stochastic Latent Transformer: Efficient Modeling of Stochastically Forced Zonal Jets},
volume = {16},
journal = {Journal of Advances in Modeling Earth Systems},
doi = {10.1029/2023MS004177}
}

@article{VpROM
author = {Simpson, Thomas and Vlachas, Konstantinos and Garland, Anthony and Dervilis, Nikolaos and Chatzi, Eleni},
year = {2024},
month = {03},
pages = {},
title = {VpROM: a novel variational autoencoder-boosted reduced order model for the treatment of parametric dependencies in nonlinear systems},
volume = {14},
journal = {Scientific Reports},
doi = {10.1038/s41598-024-56118-x}
}

@article{AutoencoderTransformer,
author = {Solera-Rico, Alberto and Sanmiguel Vila, Carlos and Gómez-López, Miguel and Wang, Yuning and Almashjary, Abdulrahman and Dawson, Scott and Vinuesa, Ricardo},
year = {2024},
month = {02},
pages = {},
title = {β-Variational autoencoders and transformers for reduced-order modelling of fluid flows},
volume = {15},
journal = {Nature Communications},
doi = {10.1038/s41467-024-45578-4}
}
